A Topic Guided Pointer-Generator Model for Generating Natural Language Code Summaries

Code summarization is the task of generating natural language description of source code, which is important for program understanding and maintenance. Existing approaches treat the task as a machine translation problem (e.g., from Java to English) and applied Neural Machine Translation models to solve the problem. These approaches only consider a given code unit (e.g., a method) without its broader context. The lacking of context may hinder the NMT model from gathering sufficient information for code summarization. Furthermore, existing approaches use a fixed vocabulary and do not fully consider the words in code, while many words in the code summary may come from the code. In this work, we present a neural network model named ToPNN for code summarization, which uses the topics in a broader context (e.g., class) to guide the neural networks that combine the generation of new words and the copy of existing words in code. Based on the model we present an approach for generating natural language code summaries at the method level (i.e., method comments). We evaluate our approach using a dataset with 4,203,565 commented Java methods. The results show significant improvement over state-of-the-art approaches and confirm the positive effect of class topics and the copy mechanism.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> architecture.tex <==
% todo: approach

% todo: supposed that our model is named as "Topic-Pointer-Generator" (need a name)
This section introduces the architecture of our method.
We first go through the overall workflow, and then the architecture details of our models, finally the main steps about dataset building and models training.

\subsection{Overall Workflow}
% overall workflow
The overall workflow of our approach is shown in Figure~\ref{fig:workflow}, which consists of two phases that are the offline training phase and the online generation phase.
It is obvious that the offline training phase aims to train LDA model and Topic-Pointer-Generator.
The online generation phase aims to generate the corresponding comment of a given method input by a user.
During the offline training phase, we uses the classes in the code corpus to train LDA model, which is then used to output top-N topics of a given method in a class.
To construct training instances for Topic-Pointer-Generator, we preprocess the classes in the code corpus including extracting methods and comments in each class and then design a training instance construction step.
During the online generation phase, the input method is first processed as a test instance that can fed into Topic-Pointer-Generator.
Then Topic-Pointer-Generator is called to generate the comment of the test instance.

% todo: overall workflow 
\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{imgs/figures-workflow}
  \caption{The workflow of approach.}
  \label{fig:workflow}
\end{figure*}

\subsection{Model Details} 
% todo
This subsection talk about the details of two important components in our architecture in Figure~\ref{fig:ourmodel}, \emph{Source Code Topic Model} and \emph{Topic-Pointer-Generator Model}.

% todo: overall architecture ？
\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{imgs/figures-net-architecture}
  \caption{Components details of architecture.}
  \label{fig:ourmodel}
\end{figure*}

\subsubsection{Get Topics via LDA model}
% model class corpus as LDA model
Given the corpus $D$ containing $M$ pieces of precessed class source code, we use LDA to model the probability of this class corpus as Equation~\ref{equ:lda} as section 3.1 mentioned.
A piece of class source code is regarded as a document containing $n$ words $d = \bm{w}_{d} = \{w_{dn}\}$.
The $N_d$ topics ${z_{dn}}$ of class source code is given by the multinomial distribution $z_{dn} \sim Multinomial(\theta_{d})$.
And each token in class source code is regard as a word $w_{dn}$ under topic $z_{dn} = k$, 
the word is given by the multinomial distribution for its topic $w_{dn} \sim Multinomial(\beta_{k})$.
% estimate and applcxxy
Given a piece of precessed class source code $d$ in the form of bag-of-words (BOW), LDA
estimate the parameters controlling the topic weights for this class source code.
Based on the topic weights of the class source code, we sort the $m$ topic weights in descending order as topics sequence $t = \{t_1, t_2, ..., t_m\}$.

\subsubsection{Generate Comment via Topic-Pointer-Generator model}
% todo pointer-generate based on topics
when generating a comment, it is general to select some tokens from input, as there is many parameters, objects and class, have their unique names, is hard for traditional network to predict. 
For this reason, we introduce pointer mechanism to solve it. 
On the other hand, To weaken the difficulty for network to search a better token in such a big vocabulary, we use topic information as a precondition and take it as another input when training our model.
So our Topic-Pointer-Generator model consist of two encoders, which support topics and source code inputs respectively. 
After being processed by LDA, we get an ordered distribution of topics for each method with their probabilities.
We select the first 10 topics as the input of topic encoder and compute a context output for each topic $(h_{1}^{topic},h_{2}^{topic},...,h_{10}^{topic})$ and a state $c_{m}^{topic}$ to represent the range information. 
Also, there is a source code encoder that receives previous state from topic encoder and the sequential source code as input. 
It also provides a context output for source code $(h_{1}^{code},h_{2}^{code},...,h_{n}^{code})$ and a state $c_{n}^{code}$. 
When decoding to an output, it will take both distributions from comment's vocabulary and source code input into consideration, across two languages. 
That's the difference from the previous pointer network. We need to compute the part of extended vocabulary $p^{extend}(y_i \mid y_1,y_2,\ldots,y_{i-1})$ for comment by taking the source code input as a query to find the inexistent tokens from comment's vocabulary, then we concatenate both extended part and previous part $p^{original}(y_i \mid y_1,y_2,\ldots,y_{i-1})$ into a final distribution $p^{final}(y_i \mid y_1,y_2,\ldots,y_{i-1})$. 
In this way, we get a unique dynamic distribution for each method.


==> implementation.tex <==
For Seq2Seq and Funcom, we use the implementations provided by~\cite{ICSE2019LeClair}.
For Funcom we implement a processor to convert source code to SBT-AO (SBT with AST only) based on the description in~\cite{ICSE2019LeClair} and concatenate source code tokens together.
%For ToPNN-PO we implement the model based on a \emph{code tokens encoder} and a decoder with pointer mechanism as mentioned before.
%For ToPNN-TO we implement the model based on a \emph{code topics encoder} and a \emph{code tokens encoder} as mentioned before, and implement the basic decoder without pointer mechanism.

For each model, the hidden size of GRU cell is set to 256, the embedding dimension for code tokens and description tokens are set to 100, and the batchsize is set to 128 due to the limitation of GPU.
For Funcom, the embedding dimension for SBT-AO is 100 which is the same to~\cite{ICSE2019LeClair}.
%For ToPNN-TO, the embedding dimension for code topics is set to 10 which is the same as setting of~\model.

We train each model for 10 epochs, and estimate BLEU metric on the validation set after each epoch.
Finally, the trained model with the best BLEU metric is chosen as the final compared model.

\app~is implemented and trained as described in Section~\ref{sec:approach}.
All the models are implemented based on Keras 2.2.4 and uses the Adam optimizer for optimizing the trainable parameters.
Each model is trained on the server with 2 Intel Xeon E5-2666v3 CPUs, 4 GTX 1080Ti GPUs, and 64G RAM which is the same as \model~training.

